Multi-Agent Relative Pose Estimation with UWB and Constrained Communications

Inter-agent relative localization is critical for any multi-robot system operating in the absence of external positioning infrastructure or prior environmental knowledge. We propose a novel inter-agent relative 2D pose estimation system where each participating agent is equipped with several ultra-wideband (UWB) ranging tags. Prior work typically supplements noisy UWB range measurements with additional continuously transmitted data, such as odometry, making these approaches scale poorly with increased swarm size or decreased communication throughput. This approach addresses these concerns by using only locally collected UWB measurements with no additionally transmitted data. By modeling observed ranging biases and systematic antenna obstructions in our proposed optimization solution, our experimental results demonstrate an improved mean position error (while remaining competitive in other metrics) over a similar state-of-the-art approach that additionally relies on continuously transmitted odometry.

==> fig/box-trial.tex <==
\begin{figure*}
    \centering
    \begin{multicols}{2}
    \begin{subfigure}{.7\linewidth}
    \includegraphics[width=\linewidth]{img/trials/box/box-traj}
    \caption{Estimated trajectory of $R_B$ wrt $R_A$}
    \label{fig:box-traj}
    \end{subfigure}
    \par
    \begin{subfigure}{\linewidth}
    \includegraphics[width=\linewidth]{img/trials/box/box-pos-err}
    \caption{Position Error vs Time}
    \label{fig:box-pos-err}
    \end{subfigure}

    \begin{subfigure}{\linewidth}
    \includegraphics[width=\linewidth]{img/trials/box/box-heading-err}
    \caption{Absolute Heading Error vs Time}
    \label{fig:box-heading-err}
    \end{subfigure}
    \end{multicols}
    
    \caption{Results from experimental trial where $R_B$ is manually driven in a box formation while $R_A$ remains static. To prevent visual clutter, only estimations from the \texttt{Raw}, \texttt{mu+Mean}, and \texttt{Weighted} algorithms are shown alongside the Vicon ground truth. Complete results can been seen in Table \mytodo{\ref{tab:pos-err} and \ref{tab:heading-err}}. (a) Shows each algorithm's 1Hz position estimation and draws an error corresponding ground truth point. (b) Shows each algorithm's position error over time for the shown trial. (c) Similarly shows each algorithm's absolute heading error for the shown trial. \mytodo{Grid lines and algorithm names}}
    \label{fig:trial-box}
\end{figure*}

==> fig/circle-trial.tex <==
\begin{figure*}
    \centering
    \begin{multicols}{2}
    \begin{subfigure}{.7\linewidth}
    \includegraphics[width=\linewidth]{img/trials/circle/circle-traj}
    \caption{Estimated trajectory of $R_B$ wrt $R_A$}
    \label{fig:circle-traj}
    \end{subfigure}
    \par
    \begin{subfigure}{\linewidth}
    \includegraphics[width=\linewidth]{img/trials/circle/circle-pos-err}
    \caption{Position Error vs Time}
    \label{fig:circle-pos-err}
    \end{subfigure}

    \begin{subfigure}{\linewidth}
    \includegraphics[width=\linewidth]{img/trials/circle/circle-heading-err}
    \caption{Absolute Heading Error vs Time}
    \label{fig:circle-heading-err}
    \end{subfigure}
    \end{multicols}
    
    \caption{\small{Results from experimental trial where $R_B$ is manually driven in a circular formation while $R_A$ remains static. To prevent visual clutter, only estimations from the \texttt{Raw}, \texttt{mu+Mean}, and \texttt{Weighted} algorithms are shown alongside the mocap ground truth. Complete results are in Table \ref{tab:pos-err} and \ref{tab:heading-err}. (a) Shows each algorithm's 1Hz position estimation and draws an error corresponding ground truth point. (b) Shows each algorithm's position error over time for the shown trial. (c) Similarly shows each algorithm's absolute heading error for the shown trial.}}
    \label{fig:trial-circle}
\end{figure*}

==> fig/weight-functions-fig.tex <==
\begin{figure*}
\centering
\begin{subfigure}{0.225\textwidth}
    \includegraphics[width=\textwidth]{img/weight-base-1}
    \caption{$w_{base,1}(x,y)$}
    \label{fig:base1}
\end{subfigure}
\hfill
\begin{subfigure}{0.225\textwidth}
    \includegraphics[width=\textwidth]{img/weight-base-2}
    \caption{$w_{base,2}(x,y)$}
    \label{fig:base2}
\end{subfigure}
\hfill
\begin{subfigure}{0.225\textwidth}
    \includegraphics[width=\textwidth]{img/weight-base-3}
    \caption{$w_{base,3}(x,y)$}
    \label{fig:base3}
\end{subfigure}
\hfill
\begin{subfigure}{0.225\textwidth}
    \includegraphics[width=\textwidth]{img/weight-base-4}
    \caption{$w_{base,4}(x,y)$}
    \label{fig:base4}
\end{subfigure}
\vfill
\begin{subfigure}{0.225\textwidth}
    \includegraphics[width=\textwidth]{img/weight-other-1}
    \caption{$w_{other,1}(x,y,\theta)$}
    \label{fig:other1}
\end{subfigure}
\hfill
\begin{subfigure}{0.225\textwidth}
    \includegraphics[width=\textwidth]{img/weight-other-2}
    \caption{$w_{other,2}(x,y,\theta)$}
    \label{fig:other2}
\end{subfigure}
\hfill
\begin{subfigure}{0.225\textwidth}
    \includegraphics[width=\textwidth]{img/weight-other-3}
    \caption{$w_{other,3}(x,y,\theta)$}
    \label{fig:other3}
\end{subfigure}
\hfill
\begin{subfigure}{0.225\textwidth}
    \includegraphics[width=\textwidth]{img/weight-other-4}
    \caption{$w_{other,4}(x,y,\theta)$}
    \label{fig:other4}
\end{subfigure}

\caption{Weight function shifted and parameterized to properly weight squared error of residual term $\tilde{z}_{ij}$.}
\label{fig:weight-function-shifted}
\end{figure*}
